Happenstance: Utilizing Semantic Search to Track Russian State Media Narratives about the Russo-Ukrainian War On Reddit

In the buildup to and in the weeks following the Russian Federation's invasion of Ukraine, Russian state media outlets output torrents of misleading and outright false information. In this work, we study this coordinated information campaign in order to understand the most prominent state media narratives touted by the Russian government to English-speaking audiences. To do this, we first perform sentence-level topic analysis using the large-language model MPNet on articles published by ten different pro-Russian propaganda websites including the new Russian "fact-checking" website waronfakes.com. Within this ecosystem, we show that smaller websites like katehon.com were highly effective at publishing topics that were later echoed by other Russian sites. After analyzing this set of Russian information narratives, we then analyze their correspondence with narratives and topics of discussion on the r/Russia and 10 other political subreddits. Using MPNet and a semantic search algorithm, we map these subreddits' comments to the set of topics extracted from our set of Russian websites, finding that 39.6% of r/Russia comments corresponded to narratives from pro-Russian propaganda websites compared to 8.86% on r/politics.

==> canned.tex <==
\begin{comment}
\begin{table}
    \small
    \centering
    \begin{tabularx}{0.5\columnwidth}{Xr}
    \toprule
     subreddit &  \# Shared Users  \\ 
    \midrule
    askreddit       &   3711 \\ 
    worldnews    &   2334 \\ 
    europe   &2166 \\
    memes & 2064 \\
    ukraines & 1852 \\
    interestingasf**k & 1844\\
    funny & 1509\\
    news & 1460\\
    gaming & 1450\\
    askarussian & 1445\\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{SubReddits with Most Shared Active Users with r/Russia}---}
   \vspace{-10pt}
    \label{table:top_link_in}
\end{table}



\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/reddit-comments-over-timepng.png}
\caption{\textbf{r/Top 10 Topics in r/Russia from Jan 1 to March 15 }--- Activity in r/Russia 
}
\label{fig:languages}
\end{figure}

\end{comment}


\begin{comment}
 


\end{comment}


\begin{comment}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{LaTeX/figures/reddit_submissions_topic_clustering.png} 
\caption{\textbf{Top topics clustered from \texttt{r/Russia} submissions}— As seen, the top topic clusters largely have little to do with Ukraine, but rather discuss a wide variety of topics ranging from Russian shows with English subtitles to talks about the harsh Russian winter. 
}
\label{figure:classification}
\end{figure}
\end{comment}


\begin{comment}
\subsection{United States News Media}
In addition to understanding attitudes and narratives towards Ukraine, we further document how the United States news media developed narratives about the Russo-Ukrainian War. In addition to helping us understand how mainstream outlets reported information about the war, this analysis also helps us perform differential analysis of the types of narratives articulated by the US mainstream outlets and the Russian state media.

Specifically, we gather 2709 different articles relating to Ukraine from eight different US online outlets across the political spectrum: nytimes.com, foxnews.com, cnn.com, washingtopost.com, reuters.com, theguardian.com, news.yahoo.com, and nbcnews.com. 


\end{comment}

\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/amount_reddit_over_time.png}
  \caption{CDF of Comments and Submissions}
\label{fig:submissions_over_time}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/deleted_comments_over_time.png}
  \caption{\% of Deleted Comments}
  \label{fig:deleted_comments}
\end{subfigure}


\begin{table}
\centering
\scriptsize
\begin{tabular}{l|r|r|r}
\hline  Domain & \#  Origin Topics  &  Avg \#  Origin Art. & Avg \# Non-Origin Art.\\ \hline
rt.com &287 & 4.97 & 3.84\\\hline 
news-front.info &287& 4.10& 2.86\\\hline 
strategic-culture.org&112 &3.02 &2.74 \\\hline 
tass &121 & 7.86& 4.14\\\hline 
katehon.com &108 &2.71&  1.86\\\hline 
geopolitica.ru &100&3.78 &2.52 \\\hline 
southfront.org &97 &5.78 &3.26\\\hline 
journal-neo.org&68  &3.21 & 2.17 \\\hline 
sputniknews.com&64  &2.56 & 2.78  \\\hline 
waronfakes.com &21 &4.71 & 2.32\\\hline 

\hline
\end{tabular}
\caption{\label{tab:real-originating}Number of topics that originated on each domain and eventually spread to at least one other domain.}  
\vspace{-0.5cm}
\end{table}


\begin{table}
\centering
\scriptsize
\begin{tabular}{l|r|r|r |r}
\hline  Domain & \# Topics & Avg \#  Art. & Avg \# External Art. & Corr.\\ \hline
rt.com & 287 & 4.97 &13.94 & ---\\\hline 
news-front.info & 216& 4.10& 17.59 & 0.525\\\hline 
strategic-culture.org & 122&3.02 & 16.59 & 0.580\\\hline 
tass & 121 & 7.86& 10.98&---\\\hline 
katehon.com & 108 &2.71& 21.32  &0.408 \\\hline 
geopolitica.ru & 100 &3.78 &18.91& 0.472 \\\hline 
southfront.org & 97 &5.78 &10.46 & --- \\\hline 
journal-neo.org & 68 &3.21 &13.21 & --- \\\hline 
sputniknews.com & 64 &2.56 & 12.30 & --- \\\hline 
waronfakes.com & 21 &4.71 &4.81 & ---\\\hline 

\hline
\end{tabular}
\caption{\label{tab:originating}Number of topics that originated on each domain and eventually spread to at least one other domain.}  
\vspace{-0.5cm}
\end{table}

\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/top_topics_04202022_map.png}
\caption{Top 10 Topics in on Russian Disinformation from Jan 1 to April 5 -- We map Russian disinformation articles to a 768 dimensional space with MPNet before utilizing UMAP to reduce the dimensionality to 2 dimensions for visualization purposes. Highlighted are the top 10 narratives identified in our dataset.
}
\label{fig:top-narrative-clusters}
\vspace{-0.5cm}
\end{figure}


\subsection{The Changing Behaviors on \texttt{r/Russia} in the Build-up to the Russo-Ukrainian War}


As seen in Figure ~\ref{fig:submissions_over_time}, immediately following Reddit's quarantine of \texttt{r/Russia}, the number of daily comments and submissions in the subreddit decreased substantially; the number of daily comments went from a seven day average of 5,168 to 118.1, and the number of daily submissions from 174.6 to 26. Reddit's quarantine effectively shut off conversation in the subreddit. We note that Reddit also banned Russian state media across their entire site as an additional step to prevent the spread of misinformation~\cite{Spangler2022}. As seen in Table~\ref{table:top_link_in}, the amount of links to our set of Russian disinformation sites is minimal. 


Despite moderation being able to largely keep hyperlinks to Russian state media articles off the platform, comments breaking community norms still managed to heavily penetrate the  \texttt{r/Russia} subreddit. As seen in  Fig~\ref{fig:deleted_comments}, a large percentage of comments were removed after they were posted on the subreddit. The large uptick in comments that did not fit the community norms of the \texttt{r/Russia} subreddit largely began during the beginning of February as Ukraine and Russia were on the verge of war. The number of comments that were deleted peaked on February 28th, the day before Reddit quarantined the subreddit, at 74.8\% of comments. 

\begin{figure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/reddit-comments-urkaine-mapped.png}
  \caption{MPNet Reddit Embeddings mapped to 2D space with Top Topics among \texttt{r/Russia} Comments in January-March 2022 highlighted.}
  \label{fig:reddit-comments-topics}
\end{subfigure}
\caption{\texttt{r/Russia} behavior at the beginning of 2022 --- As seen above, comments mentioning ``Ukraine'' and topics that associated with Ukraine and the war are bunched together in the top right of the embedding space. 
}
\label{fig:reddit_behavior}
\end{figure}


\begin{table}

\centering
\small
\begin{tabular}{l}
\toprule
\textit{Dear kids, did you know that every time you say} \\\textit{"SLAVA UKRAINE!"}\\\textit{you actually say banderites salute?}\\ \textit{Oh, have you heard about those Ukrainian heroes?} \\ \textit{You should read more about it - it\'s very fascinating reading},\\\textit{ I guarantee it!} \\ \hline
\textit{According to Ukrainian propagandists},\\ \textit{Russian Military is already destroyed,}\\ \textit{and Ukrainian Military is ready to march to Moscow...}\\ \textit{just a bit later... a bit...'}\\\hline
\textit{Zelensky said that under martial law}\\ \textit{he will allow imprisoned people with combat experience}\\ \textit{to be released to help defend Ukraine}\\
\hline
\textit{Old Russian man shot for being possible Russian}\\
\textit{saboteur breaking curfew in Ukraine.},\\ \hline

\textit{EU bans Russian media for them telling Russian point of view. }\\ \textit{Also EU: "Russia is an authoritarian country}\\\textit{ where an alternative view isn\'t an option!".}\\\textit{Wait, wait, I got it.}\\\textit{``Alternative view" means EU sponsored? Right? Right? :)}\\ 
\hline

\end{tabular}
\caption{\label{fig:narratives}Three Reddit \texttt{r/Russia} submissions made by ``freshly created`` Reddit accounts --- The \texttt{r/Russia} submissions made by freshly created accounts were highly pro-Russian and anti-Ukrainian}
\end{table}


By using a large language model and focusing on extracting topics at a sentence level, we somewhat avoid  these issues. We assume that sentences individually discuss one topic, and leverage MPNet's understanding of the English language in group together similar Russian state media sentences and Reddit comments. By mapping them to the same dimensional space, we further are able to track the set of narratives/topics addressed by Russian state-media found the most of traction on social media. 


A similar study from the RAND corporation identified two communities with 40,000 users each on Twitter that promote anti and pro-Russian narratives throughout eastern Europe. Using lexical analysis they further seek to identify relative sympathies of Twitter users to Russia as a function of their location. They find that many of the accounts spreading pro-Russian propaganda in eastern Europe were Russian in origin~\cite{helmus2018russian}. As a means of understanding the role of troll accounts (human-operated accounts tied to information operation agencies) in these seemingly non-state-sponsored campaigns, Luceri et al~\cite{luceri2020detecting}, look at classifying different Twitter users as Russian bots and trolls using clustering and an inverse reinforcement learning approach.   Finally, in Madrigal et al., researchers document the role that Facebook has had in helping to disseminate misinformation about the Russian annexation of Crimea and the 2016 Presidential election ~\cite{madrigal2017facebook}, by identifying the risk factors that prevented quick action to stop these falsehoods from reaching millions of people. 


 Gao et al. also found that by using pre-trained word embeddings and incorporating them into a Conditional Random Field regularized topic model they could get around the sparsity of short texts ~\cite{gao2019incorporating}. Bianchi et al~\cite{bianchi-etal-2021-pre} found that when performing topic analysis, utilizing large language models improved topic coherence~\cite{bianchi-etal-2021-pre}.  Peinelt et al also found that by incorporating BERT with LDA topics they could further improve upon semantic similarity tasks~\cite{peinelt2020tbert}. Huang et al~\cite{huang-etal-2021-whiteningbert-easy} found that performing unsupervised semantic analysis on the sentence level with BERT by averaging over tokens could improve results.
 
 . As a result attempting to perform topic analysis across social media posts without access to immense amounts of data is difficult and very imperfect.


\subsection{Tracking Russian Disinformation on Reddit}
On March 1, 2022, Reddit took aggressive action in quarantining the \texttt{r/Russia} subreddit. The number of comments per day on the subreddit went from thousands to tens. We find before this action, the subreddit was being bombarded by a large number of new users and Slovak-language comments. We further find that before this action several misinformation narratives expounded by the Russian State media found a home on the subreddit, with roughly between 8.3\% and 29.1\% of comments being connected to Russian state media narratives about Ukraine. We find that though the subreddit did not have a high amount of hyperlinks to Russian state media websites post moderation that many of the narratives pushed by Russian state media did find their way onto the subreddit. 




 3) Clustering and performing classed-based tf-idf on large amounts of data is heavily CPU intensive. By merely classifying the Reddit comments to the narrative clusters from newspaper articles, our approach is more generalizable and can more easily in the future accommodate identifying how millions of comments connect with articles' narratives.
 
 
We note that cosine similarity is a widely used metric in calculating embedding similarity and this similarity metric was utilized in fine-tuning the MPNet model~\cite{schnabel2015evaluation}. As noted previously amongst our topics, the average similarity score within the respective clusters was 0.56.   In this way, we attempt to understand the influence and the growth of topics identified as being spread by Russian disinformation websites on the \texttt{r/Russia} subreddit. 

 \begin{comment}
\begin{table}
    \small
    \centering
    \begin{tabularx}{0.95\columnwidth}{lrlr}
    \toprule
    Top Domain &  \# URLs &  Russian Disinfo  &  \# URLs  \\ 
    \midrule
    youtube.com       &   1925 & tass.com & 48  \\ 
    wikipedia.org    &   728 & rt.com &  36 \\ 
    imgur.com   &485 & sputniknews.com &  11 \\
    twitter.com & 294 & waronfakes.com & 2 \\
    t.me & 90&  journal-neo.org & 0  \\
    yandex.ru & 83& news-front.info & 0 \\
    github.com & 81& southfront.org &  0\\
    google.com & 70& katehon.com & 0  \\
    reuters.com & 51& geopolitica.ru & 0 \\
    bbc.com & 45 &strategic-culture.org & 0 \\
    \bottomrule
    \end{tabularx}
   \caption{Top domains and Russian disinformation websites linked by \texttt{r/Russia} between January 1 and March 15}
    \label{table:top_link_in}
\end{table}
\end{comment}

%For each of these articles, we separate each into their constituent article sentences before mapping each to our semantically rich embedding space using MPnet.  After obtaining sentence embeddings for each of our articles, we finally utilize hierarchical clustering on these sentence embeddings to separate out the various narratives present in each article. We finally run class based tf-idf ~\cite{ghosh2018class,grootendorst2020bertopic} on each cluster to obtain the descriptive keywords associated with each cluster.

\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/new_languages.png}
\caption{Language of comments on \texttt{r/Russia}. There is a large influx of Slovak language comments in the lead up to the Russo-Ukrainian War.}
\vspace{-10pt}
\label{fig:languages-over-time}
\end{figure}

\paragraph{Anti-West and NATO sentiment}
Several topics in our dataset express anti-western and anti-NATO sentiment, most notably Topic 4 and Topic 6. The North Atlantic Treaty Organization/NATO was founded in 1949 as a defensive military alliance between the United States, Canada, and several Western European countries. Largely organized against the threat of the Soviet Union, the organization adopted the agreement (Article 5) that an attack on one member of the organization would be treated as an attack on all members~\cite{NATO}. Since the fall of the Soviet Union, several new countries have joined the defensive pact including Hungary, Poland, and the Czech Republic, with North Macedonia being the newest member, leading to tensions with Russia ~\cite{NATO}. This "NATO expansionism" has been cited as one of the many causes behind the Russo-Ukrainian War in Western, Chinese  and Russian newspapers. For example, John Mearsheimer argued in The Economist, that the West's NATO expansionism provoked Russia~\footnote{\url{https://www.economist.com/by-invitation/2022/03/11/john-mearsheimer-on-why-the-west-is-principally-responsible-for-the-ukrainian-crisis}}

he dramatic uptick of new behaviors in the \texttt{r/Russia} subreddit is further mirrored in the number of \texttt{r/Russia} comments in Slovak languages, as seen in Figure~\ref{fig:languages-over-time}. Beginning in February 2022, comments in these languages came to dominate the conversation on \texttt{r/Russia}. 


Regardless of the merits of the argument of NATO expansionism as a cause of Russia's invasion, Russian newspapers and outlets have prominently weaponized this argument as a justification for the war. Russia Today, wrote 28 different articles on this subject.  Similarly Strategic Culture, a Russian think thank, wrote 27 different articles mentioning the folly of Western media converge. We see articles related to this argument throughout 2022 across every site in our dataset.   

Note, we map these comments to the narrative clusters already found by running our algorithm on Russian state media articles rather than running our full topic analysis/clustering algorithm on the Reddit and Russian state media sentences together. We do this for two reasons: 1) This allows us to be certain that the narrative clusters concern Ukraine or ideas concerning the Russo-Ukrainian. Because all \texttt{r/Russia} comments are not about Ukraine nor the Ukraine war, if we ran our full algorithm on \texttt{r/Russia} comments and our  Russian state media comments, our narrative clusters would potentially concern other topics. If a comment is not clustered or similar to Russian disinformation sentences, then we consider it an outlier and nonconnected. 2)  Our approach allows us to connect Reddit comments to the specific narratives that were known to be present in Russian disinformation campaigns. With the number of Reddit comments outweighing the number of Russian disinformation article sentences, clustering/extracting keywords from them together would inevitably give us more general clusters. Identifying which of these clusters map back to our set of original narrative clusters from Section 3 is unclear.



As seen in Figure 1, waronfakes.com (WoF), in response to the Wall Street article reporting about the potential seizure of Western companies' assets in Russia, published a story calling this article ``fake news\footnote{\url{https://web.archive.org/web/20220408201704/https://waronfakes.com/civil/fake-russian-prosecutors-office-threatened-western-companies-with-seizure-of-assets/}}.'' 


\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/wall_street_journal.jpeg}
\caption{WarOnFakes.com ``fact-checks'' the Wall Street Journal reporting that the Russian government plans to seize the assets of companies that leave the Russian market. }
\label{fig:waronfakes-examples}
\vspace{-0.5cm}

\end{figure}

Furthermore, our simplification, largely impossible without the use of large language models due to the issue of sparsity among word occurrences, enables us to understand the individual ideas present in a given set of articles.  


\begin{table}
\centering
\small
\begin{tabular}{l}
\toprule
\textit{According to Ukrainian propagandists},\\ \textit{Russian Military is already destroyed,}\\ \textit{and Ukrainian Military is ready to march to Moscow...}\\ \textit{just a bit later... a bit...'}\\\hline
\textit{Zelensky said that under martial law}\\ \textit{he will allow imprisoned people with combat experience}\\ \textit{to be released to help defend Ukraine}\\
\hline
\textit{Old Russian man shot for being possible Russian}\\
\textit{saboteur breaking curfew in Ukraine.},\\ \hline
\end{tabular}
\caption{\label{fig:narratives}Three Reddit \texttt{r/Russia} submissions made by ``freshly created`` Reddit accounts --- The \texttt{r/Russia} submissions made by freshly created accounts were highly pro-Russian and anti-Ukrainian}
\vspace{-10pt}
\end{table}




\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/prediction.drawio (1).png}
\caption{Prediction of Reddit Comments' Narrative Cluster In order to map Reddit comments to our set of news article narrative cluster, we first embed these comments to the same dimensional space with MPNet, reduce their dimensionality with UMAP, and then retrieve which narrative cluster they would have been place within using HDBScan. We then  filter out comments whose embeddings have low cosine similarity with the news articles in the cluster.}
\label{fig:topic-modeling}
\vspace{-10pt}
\end{figure}



\begin{table}
\centering
\tiny
\begin{tabular}{l|r|r|r|r}
\hline \textbf{\multirow{2}{*}{Topic}}  & \multicolumn{2}{c|}{Pre-Filter}  & \multicolumn{2}{c|}{Post-Filter} \\ \cline{2-5}
   &{\# Com.} & {Prec.} & {\# Com.}  & {Prec.}              \\   \hline 
  Topic 1  & 89 & 97.8  & 31   &  100.0                 \\ \hline
 Topic 2  & 315 & 7.6 & 10   &   70.0                  \\ \hline
  Topic 3  & 0 & ---   & 0   &  ---                 \\ \hline
 Topic 4& 599 &94.2 & 222   & 97.3  \\   \hline
  Topic 5  & 27 & 85.2  & 5   &  100                 \\ \hline
 Topic 6  & 125 & 100 & 65   & 100.0            \\   \hline    
 Topic 7 & 7 & 100 & 1   & 100.0                 \\   \hline
  Topic 8  & 109 & 95.4  & 63   &  100.0                 \\ \hline
 Topic 9  & 103 & 97.1  & 23   &  100.0                 \\ \hline
 Topic 10  & 93 & 35.4 & 10   &100.0                \\ \hline
 Topic 14  & 41 & 100 & 24   &100.0                \\ \hline
 Topic 16  & 17 & 94.1 & 1   &100.0                \\ \hline
Topic 781  & 24 & 79.2 & 18   &88.9              \\ \hline
 Topic 264  & 11 & 100 & 1   &100.0                \\ \hline
 Topic 127  & 70 & 100 & 32   &100.0                \\ \hline
  Topic 378  & 16 & 68.8 & 7   &85.7             \\ \hline
  Topic 312  & 8 & 100 & 4   &100.0                \\ \hline
   Topic 256  & 10 & 90 & 1   &100.0                \\ \hline
    Topic 500  & 4 & 100 & 0   &---             \\ \hline
    Topic 26  & 157 & 98.7 & 96  &100            \\ \hline
 \multicolumn{2}{c|}{Overall Precision}   & 77.5&  &\textbf{98.5} \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table}



\begin{figure*}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/rt.png}
  \caption{RT}
\label{fig:rt}
\end{subfigure}%
\hspace{2pt}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/sputnik.png}
  \caption{SN }
  \label{fig:sn}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/newsfront.png}
  \caption{NF}
  \label{fig:nf}
  \end{subfigure}  
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/tass.png}
\caption{Tass}
\label{fig:tass}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/sc.png}
  \caption{SC}
\label{fig:sc}
\end{subfigure}%
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/katehon.png}
  \caption{KH}
  \label{fig:kt}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/gp.png}
  \caption{GP}
  \label{fig:gp}
  \end{subfigure}  
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/jn.png}
\caption{JN}
\label{fig:jn}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/sf.png}
\caption{SF}
\label{fig:sf}
\end{subfigure}

\hspace{25pt}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/nytimes.png}
  \caption{NYT}
\label{fig:nyt}
\end{subfigure}%
\hspace{2pt}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/foxnews.png}
  \caption{FOX }
  \label{fig:fox}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/reuters.png}
  \caption{REU}
  \label{fig:reu}
  \end{subfigure}  
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/cnn.png}
\caption{CNN}
\label{fig:cnn}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/wapo.png}
  \caption{WaPo}
\label{fig:wapo}
\end{subfigure}%
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/nbc.png}
  \caption{NBC}
  \label{fig:nbc}
\end{subfigure}
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/yahoo.png}
  \caption{YH}
  \label{fig:yh}
  \end{subfigure}  
\begin{subfigure}{.10\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/guardian.png}
\caption{TG}
\label{fig:tg}
\end{subfigure}

\caption{Number of articles about a topic vs. number of Reddit comments about a topic per website--- As seen for each website, as the number of articles published about a given topic increased, so did the number of Reddit comments about that topic.
}
\label{fig:reddit_behaviorvs_russia_behavior}
\vspace{-10pt}
\end{figure*}
\begin{table}
\centering
\tiny
\begin{tabular}{l|r|r}
\hline  Domain & {0.6 \# Comm. Origin Topics} & {0.7 \# Comm.  Origin Topics} \\ \hline
rt.com & 4266 & 1191\\\hline 
news-front.info &2753 & 991\\\hline 
strategic-culture.org& 2112 &659\\\hline 
tass.com & 1141 & 313\\\hline 
katehon.com & 2072 & 739\\\hline 
geopolitica.ru & 918 & 622\\\hline 
southfront.org & 1472 &150\\\hline 
journal-neo.org&918 &237 \\\hline 
sputniknews.com&  378 & 65\\\hline 
waronfakes.com & 239 & 73\\\hline 

\hline
\end{tabular}
\caption{\label{tab:comment-topics-originating} Number of comments assigned to topic/narrative clusters that each domain originated, pre and post-filter.  }  
\vspace{-10pt}
\end{table}





We note that it is \textbf{not} the largest clusters in our dataset that had the most assigned Reddit comments. Rather the top five narratives (pre-filter) instead had 121, 9, 29, 14, and 49 articles mentioning them respectively. One of the largest topics in fact does not even have any Reddit comments assigned to it (Topic 3). Despite this initial finding, we now determine if the number the articles mentioning a given narrative/topic correlated with the number of Reddit comments about that given topic. To do so we compare the number of Reddit comments about assigned to each Russian disinformation website topic and the corresponding number of Russian disinformation website articles published about that topic. In this way, we try to ascertain the correspondence in topics that took place between Russian disinformation networks and the \texttt{r/Russia} subreddit. We do not include waronfakes.com in this analysis because it only began publishing articles (March 4, 2022) after \texttt{r/Russia}  was quarantined (March 1, 2022) when the number of comments on the\texttt{r/Russia} subreddit effectively went to 0 due to to Reddit's quarantine.


For each topic/narrative that our clustering algorithm identified, we pair this with the number of Reddit comments about that given narrative. We find that as the number of articles about a given topic increases, the number of Reddit comments increases as well with a Pearson correlation of $\rho= 0.494$ pre-filter and a Pearson correlation of $\rho=0.471$ post filter. 
The moderate correlation between and comments illustrates the degree to which the topics addressed by Russian disinformation networks mirrored those addressed by users on the \texttt{r/Russia} subreddit. While this could indicate that both Reddit and Russian disinformation networks were talking about similar ``popular'' topics regarding the war, this does illustrate the degree to which the specific narratives/topics that were pushed by Russian disinformation networks were mirrored by the \texttt{r/Russia} subreddit. In order to make sure that this phenomenon was specific to Russian disinformation websites, we ran our setup again, except this time mapping Reddit comments and topics to Western newspapers and press outlets. For this dataset, we use articles mentioning ``Ukraine'' from The New York Times (NYT, 167 articles), the Washington Post (WaPo, 174), Fox News (FOX, 123), The Guardian (TG, 158), NBC News (NBC, 131), Yahoo News (YH, 173), Reuters (REU, 200), and CNN (131) published on and before March 1,2022. We utilize the same methodology to find these articles as we utilized for our set of Russian disinformation websites. We observe a weaker correlation with the amount of articles about a topic and the number of Reddit comments increases with a Pearson correlation of $\rho= 0.297$ pre-filter and a Pearson correlation of $\rho=0.261$ post filter. This illustrates the degree to which specific Russian narratives influenced \texttt{r/Russia} rather than just popular topics. Even among comments that were not expressly deleted, we thus see that narratives and topics pushed by Russian state media enjoyed an increase in popularity in terms of the number of comments on the Reddit platform.

In particular, we observe elevated effects for several Russian disinformation websites on the r/Russia subreddit compared to other website. We plot in Figure~\ref{fig:reddit_behaviorvs_russia_behavior} the number of articles each Russian and Western Press website published about each topic against the number of Reddit comments (pre-filter) for each topic. For each website, we find as noted that as the number of articles that they wrote about a given topic increased, the number of Reddit comments increased as well. For each Western website, we again see on the whole weaker correlations than for our list of Russian disinformation websites. We find most prominently that websites like News Front ($\rho= 0.339$), Journal Neo ($\rho= 0.395$), Strategic Culture ($\rho= 0.557$), Katehon ($\rho= 0.440$), and Geopolitica($\rho= 0.450$) had the largest Pearson correlations between the number of articles that they published and the number of Reddit comments talking about the particular topic. Each of these websites had a higher correlation between their topics and Reddit comments than any Western press website. 


To ameliorate this issue, we  filter out low-cosine similar comments. After identifying a specific Reddit comment's narrative cluster, we compute the cosine similarity of its embedding with the embeddings of the newspaper sentences already in the cluster~\cite{schnabel2015evaluation}.  We then compute the average cosine similarity of the Russian disinformation media sentences within the cluster to determine if the comments' similarity is larger. We thus consider a comment to belong to a given narrative cluster if for an assigned narrative cluster $i$ with $N_i$ sentences and a potential comment $l$:
\begin{align*}
    \frac{1}{N_i} &\sum_{j}^{N_{i}} \mathbf{cos}(comment_{l}, sentence_{i,j})  \\ >  &\frac{1}{N_i}\frac{1}{N_i -1} \sum_{k\neq j}\mathbf{cos}(sentence_{i,k}, sentence_{i,j})  
\end{align*}
 After performing filtering the number of comments mapped to Russian disinformation clusters decreases to 4,455 comments (8.3\%). While the recall of our approach decreases significantly, even for topic 2 we are largely able to improve the precision of our unsupervised methodology. 
 
 
 \begin{table}
\centering
\tiny
\begin{tabular}{l|r|r}
\hline  Domain & {0.6 \# Comm. Origin Topics} & {0.7 \# Comm.  Origin Topics} \\ \hline
rt.com & 5113 & 1752\\\hline 
news-front.info &3663 & 1549\\\hline 
strategic-culture.org& 3474 &1314\\\hline 
katehon.com & 3501 & 1657\\\hline 
tass.com & 1643 & 716\\\hline 
geopolitica.ru & 1264 & 591\\\hline 
southfront.org & 1076 &319\\\hline 
journal-neo.org&1215 &438 \\\hline 
sputniknews.com&  999 & 466\\\hline 
waronfakes.com & 39 & 5\\\hline 

\hline
\end{tabular}
\caption{\label{tab:comment-topics-originating} Number of comments assigned to topic/narrative clusters that each domain originated at the comment matching similarity thresholds of 0.60 and 0.70. }  
\vspace{-10pt}
\end{table}


==> conclusion.tex <==
\section{Conclusion}

